Robusto-1 Dataset: Comparing Humans and VLMs on real out-of-distribution Autonomous Driving VQA from Peru

As multimodal foundational models start being deployed experimentally in Self-Driving cars, a reasonable question we ask ourselves is how similar to humans do these systems respond in certain driving situations -- especially those that are out-of-distribution? To study this, we create the Robusto-1 dataset that uses dashcam video data from Peru, a country with one of the worst (aggressive) drivers in the world, a high traffic index, and a high ratio of bizarre to non-bizarre street objects likely never seen in training. In particular, to preliminarly test at a cognitive level how well Foundational Visual Language Models (VLMs) compare to Humans in Driving, we move away from bounding boxes, segmentation maps, occupancy maps or trajectory estimation to multi-modal Visual Question Answering (VQA) comparing both humans and machines through a popular method in systems neuroscience known as Representational Similarity Analysis (RSA). Depending on the type of questions we ask and the answers these systems give, we will show in what cases do VLMs and Humans converge or diverge allowing us to probe on their cognitive alignment. We find that the degree of alignment varies significantly depending on the type of questions asked to each type of system (Humans vs VLMs), highlighting a gap in their alignment.

==> sec/Dataset.tex <==
\section{Dataset Overview}

The Robusto-1 Dataset is composed of \arturo{X} videos from the cities of Lima, Cusco and Cajamarca. The distribution of objects per image is the following:

\subsection{Motorized vs Non-Motorized Vehicles}

\subsection{Example use-case: Adversarial Attacks}

\subsection{Example use-case: Few-Shot learning}

An example use-case of this dataset can be few-shot learning. Earlier this year, the ROAM () organized a Challenge for participants had to (VICTOR COMPLETE HERE!). 
